Multi-Robot Path Deconfliction through Prioritization by Path Prospects

This work deals with the problem of planning conflict-free paths for mobile robots in cluttered environments. Since centralized, coupled planning algorithms are computationally intractable for large numbers of robots, we consider decoupled planning, in which robots plan their paths sequentially in order of priority. Choosing how to prioritize the robots is a key consideration. State-of-the-art prioritization heuristics, however, do not model the coupling between a robot's mobility and its environment. In this paper, we propose a prioritization rule that can be computed online by each robot independently, and that provides consistent, conflict-free path plans. Our innovation is to formalize a robot's path prospects to reach its goal from its current location. To this end, we consider the number of homology classes of trajectories, and use this as a prioritization rule in our decentralized path planning algorithm, whenever any robots enter negotiation to deconflict path plans. This prioritization rule guarantees a partial ordering over the robot set. We perform simulations that compare our method to five benchmarks, and show that it reaches the highest success rate (w.r.t. completeness), and that it strikes the best balance between makespan and flowtime objectives.

==> Figures/algorithm.tex <==
% \begin{algorithm}
% \KwData{this text}
% \KwResult{how to write algorithm with \LaTeX2e }
% \State $G \gets G_n$ %// reset graph 
% \For{$r_m \in H_n$} {
%     \State $G \gets \textsc{Trim}(G, \rho_n, V(\pi_m, \rho_m))$
% }
% \State $\pi_n \gets$ \textsc{PlanPathFromCurrentPosition}$(G, \mathbf{g}_n)$
% \Return $\pi_n$
% \caption{bla}
% \end{algorithm}



\begin{algorithm}[tb]
\caption{Dynamic Prioritized Path Planning}
\label{alg:dynamic}
\scriptsize
\begin{algorithmic}[1]
  \STATE $H_n \gets \emptyset$ // list of higher priority robots
  \STATE $L_n \gets \emptyset$ // list of lower priority robots
  \STATE $\pi_n \gets \textsc{ComputeNewPlan}(H_n)$
  %\WHILE{not at $\mathbf{g}_n$}
  \WHILE{\textsc{True}}
    \IF{new robot $r_m$ in range $c$}
        \STATE $\xi_n \gets \textsc{ComputePriority}(r_n)$
        \STATE $\textsc{BroadcastPriority}(\xi_n)$
        \STATE $\xi_m \gets \textsc{ReceivePriorityFrom}(r_m)$
        %\STATE $\textsc{UpdatePriorityLists}()$ // to reflect new $\xi_n$ and the received $\xi_m$
        \IF{$\xi_m < \xi_n$}
            \STATE $H_n \gets H_n \cup r_m$
            \STATE $\pi_n \gets \textsc{ComputeNewPlan}(H_n)$
            \STATE $\textsc{BroadcastPlan}(\pi_n)$
        \ELSIF{$\xi_m > \xi_n$}
            \STATE $L_n \gets L_n \cup r_m$
        \ENDIF
    \ELSIF{receive new priority $\xi_m$ from $r_m$}
        %\STATE // check if $r_m$ needs to be moved between $H_n$ and $L_n$
        \IF{$\xi_m < \xi_n$ \AND $r_m \in L_n$}
            %\STATE // move $r_m$ from $L_n$ to $H_n$
            \STATE $H_n \gets H_n \cup r_m$
            \STATE $L_n \gets L_n \setminus r_m$
            % \STATE $\pi_n \gets \textsc{ComputeNewPlan}(H_n)$
            % \STATE $\textsc{BroadcastPlan}(\pi_n)$
        \ELSIF{$\xi_m > \xi_n$ \AND $r_m \in H_n$ }
            %\STATE // move $r_m$ from $H_n$ to $L_n$
            \STATE $L_n \gets L_n \cup r_m$
            \STATE $H_n \gets H_n \setminus r_m$
        \ENDIF
        \STATE $\pi_n \gets \textsc{ComputeNewPlan}(H_n)$
        \STATE $\textsc{BroadcastPlan}(\pi_n)$
    \ELSIF{receive new plan $\pi_m$ from $r_m$}
        \IF{$r_m \in H_m$}
            \STATE $\pi_n \gets \textsc{ComputeNewPlan}(H_n)$
            \STATE $\textsc{BroadcastPlan}(\pi_n)$
        \ENDIF
    \ELSIF{$r_m$ left range $c$}
        \STATE $L_n \gets L_n \setminus r_m$
        \STATE $H_n \gets H_n \setminus r_m$
    \ENDIF
    
  \ENDWHILE
\end{algorithmic}

\vspace{5pt}
\textbf{Function} \textsc{ComputeNewPlan}$(H_n)$:
\begin{algorithmic}[1]
    \STATE $G \gets G_n$ // reset graph
    \FOR {$r_m \in H_n$} 
        \STATE $G \gets \textsc{Trim}(G, \rho_n, V(\pi_m, \rho_m))$
    \ENDFOR 
    \STATE $\pi_n \gets$ \textsc{PlanPathFromCurrentPosition}$(G, \mathbf{g}_n)$
    \RETURN $\pi_n$
\end{algorithmic}

% \begin{algorithm}
%  \KwData{this text}
%  \KwResult{how to write algorithm with \LaTeX2e }
%     \State $G \gets G_n$ %// reset graph 
%     \For{$r_m \in H_n$} {
%         \State $G \gets \textsc{Trim}(G, \rho_n, V(\pi_m, \rho_m))$
%     }
%     \State $\pi_n \gets$ \textsc{PlanPathFromCurrentPosition}$(G, \mathbf{g}_n)$
%     \Return $\pi_n$
% \end{algorithm}

\end{algorithm}

==> Figures/algorithm_inflation.tex <==
\begin{algorithm}
\caption{Computing Effective Obstacles}
\DontPrintSemicolon
\SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
\Input {obstacles $\mathcal{O}$, size $\rho_k$}
\Output {effective obstacles $\mathcal{O}_k$}
\label{alg:obstacles}
    $\mathcal{I} \gets \emptyset$ // set of inflated obstacles\;
    \For{$O \in \mathcal{O}$}{
        $I \gets \textsc{InflateObstacle}(\mathcal{O}, \rho_k)$ // expand the border of $O$ by $\rho_k$\;
        $\mathcal{I} \gets \mathcal{I} \cup I$\;
    }
    // transform $\mathcal{I}$ into undirected graph $\Gamma = (\mathcal{I}, E)$ where $(I_u, I_v) \in E$\;
    // if the areas of $I_u$ and $I_v$ intersect\;
    $\Gamma \gets \textsc{TransformIntoGraph}(\mathcal{I})$\;
    // compute connected components $\mathcal{C} \subseteq \mathcal{P}(\mathcal{I})$\;
    $\mathcal{C} \gets \textsc{ComputeSetsOfConnectedComponents}(\Gamma)$\;
    $\mathcal{O}_k \gets \emptyset$ // set of effective obstacles\;
    \For{$C$ in $\mathcal{C}$}{
        // $C$ is a set of overlapping obstacles\;
        $\mathcal{O}_k \gets \mathcal{O}_k \cup \textsc{MergeIntoSingleObstacle}(C)$\;
    }
    \Return $\mathcal{O}_k$
\end{algorithm}

==> sec_diversity.tex <==
%---------------------------------------------------------
\section{A Measure of Diversity}

In order to evaluate the performance of various path planning methods as a function of robot team heterogeneity, we require a function that is able to compute the \emph{diversity} of a given scenario.
Assume that a \emph{problem} is described by tuple $\mathcal{P} = \langle \mathcal{W}, \mathcal{O}, \mathcal{R}, \mathcal{A} \rangle$.
Assume also that a robot's \emph{path prospects} at time $t=0$ are given by $P_{r_i}$. Denote by $P_{\mathcal{P}} = [P_{r_i},\ldots,P_{r_n}]^\top$ a vector with the path prospects for a given problem $\mathcal{P}$. We aggregate path prospects of equal cardinality into the same class $k$, and define a proportion $\pi_k$ per class such that the sum of proportions over all classes sums to 1.
Then, using Shannon's measure of entropy, we can define a measure of \emph{path prospect diversity}
\begin{equation}
\label{eq:shannon}
    H(\mathcal{P}) = \sum_{k=1}^{K} \pi_k \log_2 \pi_k.
\end{equation}
This measure, however, does not take into account taxonomic differences between the classes $k$. For example, in a population with 2 species with equal numbers of individuals per species, the classical approach to measuring diversity is invariant with respect to the \emph{distance} between those species.
Prior work by Balch identified this shortcoming, and proposed an alternative measure to account for this~\cite{Balch:2000vi}. Balch made the key insight that a given classification of species is a function of a specific clustering level $h$, and that by varying $h$, the classifications change (and, hence, so does the diversity). Here, we make use of the alternate diversity measure termed \emph{Hierarchic Social Entropy}, since it is able to capture the distance between classes to produce a more representative measure of diversity. 
We adapt the measure proposed by Balch to our current problem formulation to propose the following diversity measure:
\begin{equation}
\label{eq:diversity}
    S(\mathcal{P}) = \int_{0}^{\infty} H(\mathcal{P}, h) dh,
\end{equation}
where $H(\mathcal{P}, h)$ corresponds to $H(\mathcal{P})$ with species (i.e., clusters) that are defined according to a given taxonomic level $h$.
Figure~\ref{fig:diversity} shows and example of two problems, one with low diversity, and one with high diversity. The dendrogram shows how the classifications aggregate into larger clusters as we increase the taxonomic level $h$.
\begin{figure}
    \centering
    \includegraphics[width=0.6\columnwidth]{Figures/empty.eps}
    \caption{Diversity of two problem variants.}
    \label{fig:diversity}
\end{figure}
